A Hamilton-Jacobi Approach for Nonlinear Model Predictive Control in Applications with Navigational Uncertainty

This paper introduces a novel methodology that leverages the Hamilton-Jacobi solution to enhance non-linear model predictive control (MPC) in scenarios affected by navigational uncertainty. Using Hamilton-Jacobi-Theoretic approach, a methodology to improve trajectory tracking accuracy among uncertainties and non-linearities is formulated. This paper seeks to overcome the challenge of real-time computation of optimal control solutions for Model Predictive Control applications by leveraging the Hamilton-Jacobi solution in the vicinity of a nominal trajectory. The efficacy of the proposed methodology is validated within a chaotic system of the planar circular restricted three-body problem.

==> To_do_list.tex <==
TO DO:

